Bayesian open games

This paper generalises the treatment of compositional game theory as introduced by Ghani et al. in 2018, where games are modelled as morphisms of a symmetric monoidal category. From an economic modelling perspective, the notion of a game in the work by Ghani et al. is not expressive enough for many applications. This includes stochastic environments, stochastic choices by players, as well as incomplete information regarding the game being played. The current paper addresses these three issues all at once.

==> lensAssociative.tex <==
\node (l1) {$(X,S)$};

\path (l1.east) -- +(1,0) node (l2)[anchor=west] {$(Y,R)$};
\path (l2.east) -- +(1,0) node (l3)[anchor=west] {$(Z,Q)$};
\path (l3.east) -- +(1,0) node (l4)[anchor=west] {$(W,T) .$};

\draw[->] (l1.east) -- node[above]{\fns$l$} (l2.west);
\draw[->] (l2.east) -- node[above]{\fns$m$} (l3.west);
\draw[->] (l3.east) -- node[above]{\fns$n$} (l4.west);
